Redundancy-Free Computation Graphs for Graph Neural Networks

Graph Neural Networks (GNNs) are based on repeated aggregations of information across nodes' neighbors in a graph. However, because common neighbors are shared between different nodes, this leads to repeated and inefficient computations. We propose Hierarchically Aggregated computation Graphs (HAGs), a new GNN graph representation that explicitly avoids redundancy by managing intermediate aggregation results hierarchically, eliminating repeated computations and unnecessary data transfers in GNN training and inference. We introduce an accurate cost function to quantitatively evaluate the runtime performance of different HAGs and use a novel HAG search algorithm to find optimized HAGs. Experiments show that the HAG representation significantly outperforms the standard GNN graph representation by increasing the end-to-end training throughput by up to 2.8x and reducing the aggregations and data transfers in GNN training by up to 6.3x and 5.6x, while maintaining the original model accuracy.

==> Makefile <==
DOC=gnn

# dependencies via include files
INCLUDED_TEX = \
  intro.tex \
  related.tex \
  model.tex \
  method.tex \
  exp.tex \

INCLUDED_FIGS =

$(DOC).pdf: $(DOC).tex bibliography.bib $(INCLUDED_TEX) $(INCLUDED_FIGS)
	pdflatex -t letter -halt-on-error $(DOC).tex
	bibtex $(DOC)
	pdflatex -t letter -halt-on-error $(DOC).tex
	pdflatex -t letter -halt-on-error $(DOC).tex

spelling :
	for f in *.tex; do aspell -p ./aspell.en.pws --repl=./aspell.en.prepl -c $$f; done


clean:
	rm -f *.bbl *.aux *.log *.blg *.lot *.lof *.dvi *.out $(DOC).pdf



==> impl.tex <==
\section{\xg Implementation}
\label{sec:impl}
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.33]{figures/impl.pdf}
%    \caption{Performance comparison among TensorFlow, DGL with PyTorch backend, and our framework. We measure the per-epoch run-time to train a 2-layer GCN model on the Pubmed dataset~\cite{GCN} on a NVIDIA Tesla V100 GPU.}
%    \label{fig:compare_impl}
%\end{figure}
Existing deep learning frameworks such as TensorFlow~\cite{Tensorflow}, PyTorch and MXNet~\cite{MXNet} are designed for spatial data structures (e.g., images and text), and have limited supports for irregular data structures such as graphs.
As a result, GNN implementations in existing frameworks translate graph structures to sparse adjacent matrices and use matrix operations to perform GNN training. 
%GNN models implemented in existing deep learning frameworks such as TensorFlow~\cite{Tensorflow}, PyTorch~\footnote{https://pytorch.org/}, and DGL~\footnote{https://dgl.ai} translate graph structures to sparse matrices and use sparse matrix operations to perform GNN operations.
This approach disables a number of critical system optimizations for graphs, such as efficient load balancing among different nodes and cache optimizations to accelerate neighborhood aggregations~\cite{Lux}, resulting in suboptimal runtime performance.

Based on the above insights we implemented our \xg abstraction in \sys, is a new deep learning framework for fast GNN training.
The key difference between \sys and existing deep learning frameworks is that \sys explicitly manages graph structures in GNNs and reduces GNN training to a number of graph processing operations, such as node gather/scatter operations.

The aggregations in each GNN layer are reduced to a global node scatter operation, which scatters the previous-layer activations of each node (i.e., $h^{(k-1)}_v$) along the edge direction, and a global node gather operation, which aggregates the neighbors of each node by gathering in-edges.

The updates in each GNN layer are reduce to a global node update operation, which computes the new activations of each node (i.e., $h^{(k)}_v$).

\sys can directly benefit from various existing system optimizations for graphs.
We implemented \sys on top of Lux~\cite{Lux}, a high-performance graph processing framework, and used cuDNN~\cite{cudnn} and cuBLAS~\cite{cublas} as the underlying libraries to perform tensor operations such as matrix multiplications.

%We implemented our GNN framework in Lux~\cite{Lux}, a high-performance graph processing framework.
Figure~\ref{fig:compare_training} compares the training performance of TensorFlow, DGL with PyTorch, and \sys and shows that \sys significantly outperforms existing frameworks that use sparse matrix operations to perform GNN training.
The speedup is due to a number of system optimizations enabled by maintaining graph structures in \sys.

It is worth noting that our framework uses the same program interface as DGL, and therefore existing GNNs can directly run on our framework without any changes to the GNNs.



==> model.tex <==
\section{Graph Neural Network Abstraction}
\begin{algorithm}[t]
\caption{An abstraction for GNNs. $\mathcal{V}$ is the set of nodes in an input graph, and $\mathcal{N}(v)$ denotes the set of neighbors for node $v$.}
\label{alg1}
\begin{algorithmic}[1]
\State $h^{(0)}_v = x_v, \forall v \in \mathcal{V}$
\For {$k= 1 \textrm{ to } K$}
\For {$v \in {\mathcal{V}}$}
\State $a^{(k)}_v \leftarrow \Call{Aggregate}{\{h^{(k-1)}_u | u \in \mathcal{N}(v)\}}$
\State $h^{(k)}_v \leftarrow \Call{Update}{a^{(k)}_v, h^{(k-1)}_v}$
\EndFor
\EndFor
\State
\State {\bf Goal:} minimize $\mathcal{L}(\{h^{(K)}_v | v \in \mathcal{V}\})$
\end{algorithmic}
\end{algorithm}
A GNN takes an input graph and node features as inputs and iteratively learns representations for individual nodes over the entire graph through a number of GNN layers.
%Each GNN layer consists of two steps.
Algorithm~\ref{alg1} shows an abstraction for GNNs: $h^{(k)}_v$ is the learned activations of node $v$ at layer $k$, and we initialize $h^{(0)}_v$ with input node features $x_v$.
At the $k$-th layer, $a^{(k)}_v$ denotes the aggregated activations of $v$'s neighbors, which is combined with $h^{(k-1)}_v$ to compute an updated activation $h^{(k)}_v$.
The learned node activations of the final layer (i.e., $h^{(K)}_v$) are used for predictions, and a GNN model generally minimizes a loss function $\mathcal{L}$ that takes the final node activations as inputs (line 7).

\begin{table*}[t]
\caption{Existing GNNs described in our abstraction. GraphSAGE-P and GraphSAGE-LSTM are the pooling and LSTM variants of GraphSAGE, respectively. $\sigma$ and $\er{max}$ indicate element-wise non-linear activation and max functions.
For sequential \textproc{Aggregate}, $v_i$ denotes the $i$-th in-neighbor of node $v$.
}
\label{tab:gnns}
\begin{threeparttable}
\resizebox{\textwidth}{!}{
\begin{tabular}{lll}
\hline
{\bf GNN} & {\bf $\textproc{Aggregate}(\{h^{(k-1)}_u | u \in \mathcal{N}(v)\})$} & {\bf $\textproc{Update}(a^{(k)}_v, h^{(k-1)}_v)$}\\
\hline
\multicolumn{3}{c}{Set \textproc{Aggregate}} \\
\hline
GCN~\cite{GCN} & $a^{(k)}_v = \sum_{u\in\mathcal{N}(v)}{h^{(k-1)}_u} $ & $h^{(k)}_v = \sigma(W^{(k)} \cdot \frac{a^{(k)}_v + h^{(k-1)}_v}{|\mathcal{N}(v)| + 1})$ \\
%GIN~\cite{GIN} & $a^{(k)}_v = \sum_{u\in\mathcal{N}(v)}{h^{(k-1)}_u} $ & $h^{(k)}_v = \sigma\big(W \cdot \Big((1 + \epsilon^{(k)})h^{(k-1)}_v + a^{(k)}_v\big) \Big)$ \\
GraphSAGE-P~\cite{GraphSAGE} & $a^{(k)}_v = {\er{max}}_{u\in\mathcal{N}(v)}\{\sigma(W^{(k)}_1 \cdot h^{(k-1)}_u)\}$ & $h^{(k)}_v = \sigma\big(W^{(k)}_2 \cdot (a^{(k)}, h^{(k-1)}_v)\big)$ \\
%GraphSAGE~\cite{GraphSAGE} & $a^{(k)}_v = \frac{1}{|\mathcal{N}(v)|}\sum_{u\in\mathcal{N}(v)}{h^{(k-1)}_u}$ & $h^{(k)}_v = \sigma\big(W^{(k)} \cdot (a^{(k)}_v, h^{(k-1)}_v)\big)$\\
%\hline
%\multicolumn{3}{c}{Idempotent \textproc{Aggregate}} \\
%\hline
%GCN-P~\cite{GCN} & $a^{(k)}_v = {\er{max}}_{u\in\mathcal{N}(v)}\{h^{(k-1)}_u\} $ & $h^{(k)}_v = \sigma\big(W^{(k)} \cdot (a^{(k)}_v | h^{(k-1)}_v)\big)$ \\
\hline
\multicolumn{3}{c}{Sequential \textproc{Aggregate}} \\
\hline
GraphSAGE-LSTM~\cite{GraphSAGE} & $a^{(k)}_v = \er{LSTM}(h^{(k-1)}_{v_1},...,h^{(k-1)}_{v_\mathcal{N}})$ & $h^{(k)}_v = \sigma\big(W^{(k)} \cdot (a^{(k)}_v, h^{(k-1)}_v)\big)$\\
$N$-ary Tree-LSTM~\cite{TreeLSTM} & $a^{(k)}_v = \er{Tree-LSTM-Agg}(h^{(k-1)}_{v_1},...,h^{(k-1)}_{v_\mathcal{N}})$ & $h^{(k)}_v = \er{Tree-LSTM-Update}(a^{(k)}_v, h^{(k-1)}_v)$\\
\hline
\end{tabular}
}
\end{threeparttable}
\end{table*}



